Graph Convolutional Embeddings for Recommender Systems

Modern recommender systems (RS) work by processing a number of signals that can be inferred from large sets of user-item interaction data. The main signal to analyze stems from the raw matrix that represents interactions. However, we can increase the performance of RS by considering other kinds of signals like the context of interactions, which could be, for example, the time or date of the interaction, the user location, or sequential data corresponding to the historical interactions of the user with the system. These complex, context-based interaction signals are characterized by a rich relational structure that can be represented by a multi-partite graph. Graph Convolutional Networks (GCNs) have been used successfully in collaborative filtering with simple user-item interaction data. In this work, we generalize the use of GCNs for N-partite graphs by considering N multiple context dimensions and propose a simple way for their seamless integration in modern deep learning RS architectures. More specifically, we define a graph convolutional embedding layer for N-partite graphs that processes user-item-context interactions, and constructs node embeddings by leveraging their relational structure. Experiments on several datasets from recommender systems to drug re-purposing show the benefits of the introduced GCN embedding layer by measuring the performance of different context-enriched tasks.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.


==> acknowledgement.tex <==
\vspace{0.3cm}
\noindent\textbf{Acknowledgements}. The GPUs used in this research are provided by NVIDIA Corporation with 1080Ti series. This research is supported by the Thousand Youth Talents Program 2018. Joemon Jose and Xiangnan He are corresponding authors.
%We also gratefully acknowledge the support of NVIDIA Corporation with the donation of the Titan Xp GPU used for this research.

==> reviews.tex <==
Thank you for submitting your work to WSDM 2021. We regret to inform you that your submission below was not selected for the WSDM 2021 conference:

Submission 232: Graph Convolutional Embeddings for Recommender Systems

This year we received 603 submissions. We were able to accept only 112 of these, representing an acceptance rate of 18.6%. Due to the limited number of available slots in the conference schedule, we unfortunately had to make very difficult decisions and decline many submissions.

The program committee worked very hard to thoroughly review all the submitted papers, and to provide suggestions to improve your paper. All papers were reviewed by at least three program committee members, and by at least one senior PC member to oversee discussion amongst the reviewers and provide an overall recommendation for the paper. Please find the reviews for your paper below.  We hope these will be useful to revise your work for future submissions.

While we understand that this outcome may be disappointing, we hope that you will still consider attending the conference. 

Best regards,
Eugene Agichtein and Evgeniy Gabrilovich
WSDM 2021 Program Co-Chairs

SUBMISSION: 232
TITLE: Graph Convolutional Embeddings for Recommender Systems

-------------------------  METAREVIEW  ------------------------
This paper received scores -1, -1, 0, 0.  Based on the reviews, my recommendation is to reject.  There are several concerns regarding the experiments, including one concern around the results for Frappe and how to understand them, and a related concern that the places where GCE performs well are not well-explained in the paper (perhaps Xu et al can be used as an example of a mechanism to study expressive power, as suggested in review 4).  Finally, there is a concern expressed in review 3 that the algorithmic idea combines existing techniques, but does not in itself bring sufficient novelty.



----------------------- REVIEW 1 ---------------------
SUBMISSION: 232
TITLE: Graph Convolutional Embeddings for Recommender Systems
AUTHORS: Paula Gomez, Alexandros Karatzoglou, Xin Xin and Ioannis Arapakis

----------- Strengths -----------
* Context-aware recommendation is an interesting and important problem.
* Extending GCN to model N-partite graph in context-aware recommender systems is a nice try.
* The experimental results show that the proposed method can improve the performances of FM baseline.
----------- Weaknesses -----------
* Experiments are somewhat weak and not convincing.
1. Some important baselines missing in the experiments, like lightGCN [1], NGCF, or other context-aware recommendation baselines. Although the experimental results shows the proposed graph convolutional embedding can improve FM results, we still do know how it performs when comparing with other strong GNN baselines like lightGCN.
2. Results in Table 4 show that GCE layer is not alway helpful for downstream models. For results in Table 2, the authors' explain, "the second order connectivity effects on this graph are already captured in some form by other deeper models", is not persuasive. If the second order connectivity effects are already captured, then first-order connectivity effects should also be captured. Then, why does GCE-DFM still work? It is unlikely that DFM only encodes the second-order connectivity while omits first-order connectivity.
3. From the paper, it is not clear whether context information is leveraged in the baselines or not? It looks like the baselines do not use the context information. If so, then it is unclear the improvements in results come from more input features or the proposed GCE layer.

[1] Xiangnan He, Kuan Deng, Xiang Wang, Yan Li, Yongdong Zhang and Meng Wang. LightGCN: Simplifying and Powering Graph Convolution Network for Recommendation. SIGIR 2020
----------- Paper Clarity -----------
SCORE: 4 (good: most of the paper was understandable, with minor typos or details that could be improved)
----------- Significance -----------
SCORE: 3 (Moderate advance in methodology or understanding of phenomena, likely to be useful to others)
----------- Interest to Audience -----------
SCORE: 4 (Interesting to many attendees)
----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
This paper proposed to use GCN as an embedding layer in the downstream recommendation model for processing generalized user-item-context interactions.
Extending GCN to model N-partite graph in context-aware recommender systems is a nice try.
However, the experiments are somewhat weak and not convincing.
Besides, more analysis experiments need to be conducted to answer how and why does the proposed GCE work? 


some detail comments:
* Equation 3 is wrong. $W$ should be placed in brackets
* Citation 24 is not complete.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 232
TITLE: Graph Convolutional Embeddings for Recommender Systems
AUTHORS: Paula Gomez, Alexandros Karatzoglou, Xin Xin and Ioannis Arapakis

----------- Strengths -----------
1) Generalizing the use of Graph Convolutional Network as embedding layers for Recommender Systems.
2) Making Recommender Systems to use contextual information in presence of N-partite graphs - to capture higher order non-linear interaction signals.
3) Integration with downstream recommendation models
4) Information about code and datasets are provided to aid reproducibility
----------- Weaknesses -----------
1) GCN is employed in the recommender systems to address user-item-context interactions yet it seems not to achieve uniformly better results in context-aware dataset Frappe.
2) GCE layers formed using GCNs are claimed here to be generalizable - why restrict to Recommender systems? other areas of application could be discussed to bring out the broad advantages of this approach.
3) Related works are discussed fairly, but need to compare and evince more on how the proposed approach is distinctive from the rest of existing works.
----------- Paper Clarity -----------
SCORE: 3 (average: the main points of the paper was understandable, but some parts were not clear)
----------- Significance -----------
SCORE: 2 (Minor or incremental advance over known techniques or insights)
----------- Interest to Audience -----------
SCORE: 3 (Some interest to a large fraction of the attendees or alot of interest to some)
----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
The paper brings novelty by applying GCNs as embedding layers for recommender systems and also suggests ideas to overcome data sparsity through employing concepts such as Multi-hop convolution. 
The paper provides evidence for the proposed architecture that is based on GCN's message passing principle, using Factorization Machines (NFM, DFM and WD) and its variants as the base model and the experiments were conducted over four different benchmark datasets namely: MovieLens-1M, nowplaying-RS, User-Book Interactions, and Frappé.
More experimental comparisons with most closely related works stated are missing. Especially the models that focus only on bipartite user-item interactions such as GC-MC.
Need to showcase the performance of GCE over datasets dedicated for context-aware interactive information.
Finally, the paper could use a bit of re-organization - too much low-level details are discussed in the Related works sections making the reader to lose track of the paper's contribution in light of existing works, and also minor typos exist like under section 3.3.

Recommending a weak reject.



----------------------- REVIEW 3 ---------------------
SUBMISSION: 232
TITLE: Graph Convolutional Embeddings for Recommender Systems
AUTHORS: Paula Gomez, Alexandros Karatzoglou, Xin Xin and Ioannis Arapakis

----------- Strengths -----------
1.  The paper creates a graph convolutional embedding layer that can process user-item-context interactions , it can be used in downstream recommendation tasks.

2.  The paper proposes to use multi-hop propagation in one GCE layer to reduce the number of parameters.

3. The description of experimental design and technical details is clear described.
----------- Weaknesses -----------
1.  The GCE adds a lot of user-item-context interaction, time and memory cost need to be compared, but no comparative experiments are designed in the experiment section.

2.  The paper says:’’ combining GCE with several stateof-the-art recommendation models’’, the baselines it chose (FM2010, DFM2017, NFM2017) are not the latest. There are some other models that can be used as baselines, e.g. xDeepFM. 

3.  The paper[1] may be related to graph convolutional embeddings. The author should explain the differences and  connections between them and whether they need to be compared?
[1] Chen, Chih-Ming, et al. "Collaborative Similarity Embedding for Recommender Systems." International World Wide Web Conferences abs/1902.06188 (2019): 2637-2643.

4. There are some descriptions in the paper that are not clear, which is difficult to understand. For example, 
What do implicit and explicit  mean in the last paragraph of Introduction? The description of N is inconsistent
 in Section 2.2 and 3.1.
----------- Paper Clarity -----------
SCORE: 3 (average: the main points of the paper was understandable, but some parts were not clear)
----------- Significance -----------
SCORE: 3 (Moderate advance in methodology or understanding of phenomena, likely to be useful to others)
----------- Interest to Audience -----------
SCORE: 2 (Interesting to a small group or sub-specialty)
----------- Overall evaluation -----------
SCORE: 0 (borderline paper)
----- TEXT:
In order to model the context of user-item interaction in the area of recommender systems, this paper generalizes GCNs to both arbitrary multiple context dimensions and also integrates it into the RS model to improve the performance of downstream tasks. The experimental results also show that this method is more effective than some traditional methods in several datasets. The paper is easy to understand and has detailed method descriptions. The entire experiment is relatively complete, which introduces the statistics of the datasets, hyperparameters setting, experiment analysis , and comparison baselines. 

Compared with the previous methods, GCE considers more contextual interaction, but the modeling method and implementation process are still the original methods. This idea is not innovative enough.  

In the experimental part, GCE needs to be integrated and tested with the latest RS model to prove its effectiveness. In more complex context interactions, GCE will focus on more user-item-context interaction, which may limit its practical application. Therefore, the paper needs to consider the additional cost of introducing a lot of interaction context, and illustrates it through time or memory cost. 

There are also some grammatical errors and missing technical details in the paper (e.g., S_ei in Eq.(1) ).  

This paper lacks some comparisons of related work. For example, in the experimental part, the model comparison only has GCE and its extension method (GCE-hop), and other embedding methods should be added. In summary, my opinion is 0 (borderline paper).



----------------------- REVIEW 4 ---------------------
SUBMISSION: 232
TITLE: Graph Convolutional Embeddings for Recommender Systems
AUTHORS: Paula Gomez, Alexandros Karatzoglou, Xin Xin and Ioannis Arapakis

----------- Strengths -----------
1.      The proposed model is compatible with any downstream recommendation models
2.      The proposed model can be generalized to deal with arbitrary multiple context dimensions
3.      The experimental results show the effectiveness of expressive power of repeated graph convolution operation in three out of four datasets
----------- Weaknesses -----------
1.      The proposed model is quite straightforward in its formulation, and contribution is limited. 
2.      The experimental validation is lacking in many aspects. I expect the authors can provide more thorough analysis based on the results as well as comparison with some other GCN-based recommender systems.
----------- Paper Clarity -----------
SCORE: 3 (average: the main points of the paper was understandable, but some parts were not clear)
----------- Significance -----------
SCORE: 3 (Moderate advance in methodology or understanding of phenomena, likely to be useful to others)
----------- Interest to Audience -----------
SCORE: 3 (Some interest to a large fraction of the attendees or alot of interest to some)
----------- Overall evaluation -----------
SCORE: 0 (borderline paper)
----- TEXT:
This work presents a generalized GCN encoder is highly efficient and can handle arbitrary number of contexts. The resulting embeddings are compatible with any downstream recommendation model. The main contribution is to handle user-item-context information by using existing GCN approach and produce embeddings for existing factorization methods. Overall, it’s an interesting paper, but there are some flaws.

1. They applied GCE layer into four factorization methods. However, they did not compare their approach against original GCN methods for recommendation. What if factorization with GCE produce lower performance than other GCN methods? I would suggest them to add additional baselines.

2. They chose four factorization methods which were published in 2017 or before 2017. Does this mean there is no recent recommendation methods to handle user-item-context info? Why don’t you add recent baselines to see whether adding GCE still produce similar improvements.

3. The experimental results show the effectiveness of the GCE layer, but, they did not clearly deliver detailed insights why it performed better. As the expressive power has been studied theoretically by previous work [1], it would be better if the authors can provide more concrete analysis.
[1] Xu, K., Hu, W., Leskovec, J., & Jegelka, S. (2018). How powerful are graph neural networks?. arXiv preprint arXiv:1810.00826.

4. In Frappe dataset, GCE layer did not produce improvements in NDCG for FM, NFM and DFM. The current explanation is not clear/persuasive. I encourage them to further analyze why it is not boosting the performance and actually degrading performance.




